Analysing Factorizations of Action-Value Networks for Cooperative Multi-Agent Reinforcement Learning

Recent years have seen the application of deep reinforcement learning techniques to cooperative multi-agent systems, with great empirical success. However, given the lack of theoretical insight, it remains unclear what the employed neural networks are learning, or how we should enhance their learning power to address the problems on which they fail. In this work, we empirically investigate the learning power of various network architectures on a series of one-shot games. Despite their simplicity, these games capture many of the crucial problems that arise in the multi-agent setting, such as an exponential number of joint actions or the lack of an explicit coordination mechanism. Our results extend those in [4] and quantify how well various approaches can represent the requisite value functions, and help us identify the reasons that can impede good performance, like sparsity of the values or too tight coordination requirements.

==> table.tex <==
\footnotesize

\pgfplotstableset{
begin table=\begin{longtable},
alias/Model/.initial=0,
end table=\caption{Accuracy results for the different games.}
\label{tab:measures}
\end{longtable}
\clearpage
}

\rowcolors{2}{lightgray!50}{}

\pgfplotstabletypeset[col sep=comma,
	every head row/.style={before row=\toprule},
    every last row/.style={after row=\bottomrule},
	header=false,
	fixed,
	zerofill,
    columns/Model/.style={column type={C{0.55cm}},string type},
	columns/Mean square error/.style={string type, column type={C{1.2cm}}},
	create on use/Mean square error/.style={
		create col/assign/.code={
		\pgfmathprintpmnumber{1}{2}{2}{1}
		\pgfkeyslet{/pgfplots/table/create col/next content}\value
		}
	},
	columns/MSE on optimal actions/.style={string type, column type={C{1.2cm}}},
	create on use/MSE on optimal actions/.style={
		create col/assign/.code={
		\pgfmathprintpmnumber{3}{4}{2}{1}
		\pgfkeyslet{/pgfplots/table/create col/next content}\value
		}
	},
	columns/Optimal actions found/.style={string type, column type={C{0.9cm}}},
	create on use/Optimal actions found/.style={
		create col/assign/.code={
		\pgfmathprintpmnumber{5}{6}{0}{0}
	    \pgfkeyslet{/pgfplots/table/create col/next content}\value
		}
	},
	columns/Value loss/.style={string type, column type={C{1.5cm}}},
	create on use/Value loss/.style={
		create col/assign/.code={
		\pgfmathprintpmnumber{7}{8}{2}{1}
		\pgfkeyslet{/pgfplots/table/create col/next content}\value
		}
	},
	columns/Boltzmann value loss/.style={string type, column type={C{1.5cm}}},
	create on use/Boltzmann value loss/.style={
		create col/assign/.code={
		\pgfmathprintpmnumber{9}{10}{2}{1}
		\pgfkeyslet{/pgfplots/table/create col/next content}\value
		}
	},
	columns/Correctly ranked/.style={string type, column type={C{1.5cm}}},
	create on use/Correctly ranked/.style={
		create col/assign/.code={
		\pgfmathprintpmnumber{11}{12}{0}{0}
		\pgfkeyslet{/pgfplots/table/create col/next content}\value
		}
	},
	columns/Kendall Tau/.style={string type, column type={C{1.1cm}}, column name={Kendall $\tau$}},
	create on use/Kendall Tau/.style={
		create col/assign/.code={
		\pgfmathprintpmnumber{13}{14}{2}{1}
		\pgfkeyslet{/pgfplots/table/create col/next content}\value
		}
	},
	columns={Model,Mean square error,MSE on optimal actions,Optimal actions found,Value loss,Boltzmann value loss,Correctly ranked,Kendall Tau},
	every row no 0/.style={before row={\midrule\multicolumn{8}{c}{\textbf{Dispersion game (64 joint actions, 20 optimal)}}\\\midrule}},
	every row no 15/.style={before row={\midrule\multicolumn{8}{c}{\textbf{Platonia dilemma (64 joint actions, 6 optimal)}}\\\midrule}},
	every row no 30/.style={before row={\midrule\multicolumn{8}{c}{\textbf{Climb game (729 joint actions, 1 optimal)}}\\\midrule}},
	every row no 45/.style={before row={\midrule\multicolumn{8}{c}{\textbf{Penalty game (729 joint actions, 2 optimal)}}\\\midrule}},
	every row no 60/.style={before row={\midrule\multicolumn{8}{c}{\textbf{Generalized firefighting (8192 joint actions, 779 optimal)}}\\\midrule}},
	every row no 75/.style={before row={\midrule\multicolumn{8}{c}{\textbf{Aloha (64 joint actions, 2 optimal)}}\\\midrule}},
]{csv/Combined.csv}
